Minimizing Total Busy Time with Application to Energy-efficient Scheduling of Virtual Machines in IaaS clouds

Infrastructure-as-a-Service (IaaS) clouds have become more popular enabling users to run applications under virtual machines. Energy efficiency for IaaS clouds is still challenge. This paper investigates the energy-efficient scheduling problems of virtual machines (VMs) onto physical machines (PMs) in IaaS clouds along characteristics: multiple resources, fixed intervals and non-preemption of virtual machines. The scheduling problems are NP-hard. Most of existing works on VM placement reduce the total energy consumption by using the minimum number of active physical machines. There, however, are cases using the minimum number of physical machines results in longer the total busy time of the physical machines. For the scheduling problems, minimizing the total energy consumption of all physical machines is equivalent to minimizing total busy time of all physical machines. In this paper, we propose an scheduling algorithm, denoted as EMinTRE-LFT, for minimizing the total energy consumption of physical machines in the scheduling problems. Our extensive simulations using parallel workload models in Parallel Workload Archive show that the proposed algorithm has the least total energy consumption compared to the state-of-the art algorithms.

==> approximations.tex <==
% % File: approximations.tex
% % Approximation of some special cases

\subsection{Approximation algorithm for general case}
\label{sec:approxgenerlcase}
 
In this section, we claim that algorithm EMinTRE-LFT for general instance yields its approximation ratio are $g$, 
 where $g$ is the maximal number of virtual machines can be assigned to each physical machine.
%\khanh{not clear???}
 EMinTRE-LFT sorts the list of virtual machines in order of their longest duration time first.
 
 \begin{theorem}
 	For any instance $\Ja$, EMinTRE-LFT is a $g$-approximation algorithm where $g$ is the maximal number of virtual machines can be assigned to each physical machine, i.e. 
 	the total busy time of schedule for $\Ja$ outputted by EMinTRE-LFT is the maximum $g$ times the total busy time of optimal schedule. 
 	We denote $EMinTRE-LFT(\Ja)$ is cost of algorithm EMinTRE-LFT for a given instance $\Ja$ that is defined in the \ref{def:costalg}.
 	Formally, 
 	\begin{equation}
 		EMinTRE-LFT(\Ja) \leq g \cdot OPT(\Ja).
 	\end{equation}
 \end{theorem}
 
 \begin{proof}
 	Let $N(t)$ denote the number of virtual machines that could be placed at time $t$. Let $N^{H}(t)$ denote the number of used physical machines at time $t$ in a schedule that is resulted by algorithm EMinTRE-LFT,
 	%are the number of physical machines that are output in schedule that made by the proposed EMinRET algorithm at time $t$, 
 	%Let $N^{H}(t)$ denotes the number of used physical machines at time $t$ in the schedule output by the algorithm, 
 	and $N^{OPT}(t)$ denotes the number of machines used at time $t$ in an optimal schedule.
 	
 	For any time $t \geq 0$, each of using $N^{H}(t)$ physical machines has at least one allocated virtual machine, i.e.,
 	$N(t) \geq N^{H}(t)$. 
 	Clearly, at any time $t \geq 0$ and $g \geq 1$, $N^{OPT}(t) \geq \frac{N(t)}{g} = \frac{N^{H}(t)}{g}$. 
 	 	 	
 	The total busy time of the entire schedule of an instance $\Ja$ denoted as $EMinTRE-LFT(\Ja)$ is calculated by taking the integral of $N^{H}(t)$ with all values of $t \in [0, span(\Ja)]$. Thus, we have:
 	
 		$N^{OPT}(t) \geq \frac{N^{H}(t)}{g}$
 		$\Longleftrightarrow N^{H}(t) \leq g \cdot N^{OPT}(t)$ \\
 		
 		$\Rightarrow \int\limits_{0}^{span(\Ja)} N^{H}(t) dt \leq g \cdot \int\limits_{0}^{span(\Ja)} N^{OPT}(t) dt$\\
 		
 		$\Longleftrightarrow EMinTRE-LFT(\Ja) \leq g \cdot OPT(\Ja) $ \\
 		
% 		$\Longleftrightarrow \frac{EMinTRE-LFT(\Ja)}{OPT(\Ja)} \leq g$

	Thus, by applying the same reasoning to other algorithms such as EMinTRE-LFT, we have:
	
	$EMinTRE-LFT(\Ja) \leq g \cdot OPT(\Ja) $ 
	%% The theorem is proved.
 \end{proof}
 


==> fig-algo.tex <==
\begin{algorithm*}[!hbt]
\caption{EMinRET-ST and EMinRET-FT: Heuristics for energy-aware VM allocation in HPC Clouds}\label{alg:remindft}
\begin{algorithmic}[1]

\Function{EMinRET-ST}{}
\State	\textit{Input:} vmList - a list of virtual machines to be scheduled
\State	\textit{Input:} hostList - a list of physical servers
\State	\textit{Output:} mapping (a feasible schedule) or null % \khanh{should be ``null''?. OK}
\State	vmList = sortVmListByStartTime( vmList ) \Comment{1}\label{line:sortbystarttime}
\State return EMinRET( vmList, hostList )
\EndFunction

\Function{EMinRET-FT}{}
\State	\textit{Input:} vmList - a list of virtual machines to be scheduled
\State	\textit{Input:} hostList - a list of physical servers
\State	\textit{Output:} mapping (a feasible schedule) or null % \khanh{should be ``null''?. OK}
\State	vmList = sortVmListByFinishTime( vmList ) \Comment{2}\label{line:sortbyfinishtime}
\State return EMinRET( vmList, hostList )
\EndFunction

\end{algorithmic}
\end{algorithm*}



==> problem-constraints.tex <==
%The scheduling problem has the following hard constraints that are described in our previous work \cite{HungFDSE2014}.
The scheduling problem has the following hard constraints, which are firstly described in our previous work \cite{HungFDSE2014}, as following:
\begin{itemize}
\item Constraint 1: Each VM is only processed by a physical server at any time with non-migration and non-preemption.

\item Constraint 2: %Every virtual machine do not request any resource larger than the maximum total capacity of resource in any host.
Each VM does not request any resource larger than the maximum total capacity resource of any physical server.

\item Constraint 3: %Let $n_{j}(t)$ be the set of indexes of VMs that are allocated onto $M_{j}$ at time $t$. 
The sum of total demand resources of these allocated VMs is less than or equal to the total capacity of the resources of $M_j$.
Each VM is represented
as a $d$-dimensional vector of demand resources, 
i.e. $vm_{i} = (x_{i,1}, x_{i,2}, ..., x_{i,d}) $.
Similarly,
each physical machine is denoted as a d-dimensional 
vector of capacity resources, 
i.e. $ M_{j} = (y_{j,1}, y_{j,2}, ...,  y_{j,d}) $. Thus we have
$\forall r \in \{1,...,d\}, i \in \{1,2,...,n\}, j \in \{1,2,...,m\}:$
\end{itemize}

\begin{equation}
%% \sum\limits_{vm_{i} \in r_{j}(t), t \in T_j} x_{i,c} \leq y_{j,c}
\sum\limits_{vm_i \in \Ja_{j}} x_{i,r} ~~~~~~~\leq ~~~~~~~ y_{j,r}
\end{equation}


{\noindent} where:

- $x_{i,r}$ is resource of type $r$ (e.g. CPU core, computing power, memory, etc.) requested by the $vm_{i}$ (i=1,2,...,n).

- $y_{j,r}$ is capacity resource of type $r$ (e.g. CPU core, computing power, memory, etc.) of the physical machine $M_{j}$ ($j=1,2,...,m$).


%Even if all physical servers are identical and all VMs are identical too,
With at least one type of resource (i.e., $d \ge 1$), the scheduling problem is NP-hard \cite{Panigrahy2011}.
%We assume that the power consumption model is linear to CPU utilization.
%\todo{HUNG: linearly as in equation (1)}
%\khanh{I got it. This paragraph needs to rephase since it is repetitive (consider later - edit writing)}
%With the problem considered in this paper,
%all physical servers are identical and 
%their power consumption models are linear to their CPU utilization
%as can be seen in the two equations (\ref{eq:power}) and (\ref{eq:energy}).
%The energy consumption of a physical server in a time unit is denoted as $E_{0}$
%and is the same for all physical servers since the servers are identical.
%\khanh{how to compute $E_0$?}\hung{$E_0$ is same as P^{idle}}


%In this paper, we use the following energy consumption model proposed in \cite{Quang-hung2015} for a physical machine.


==> referenc.tex <==
\begin{thebibliography}{4}

%\bibitem{Albers2010} Albers, S. and Fujiwara, H.: Energy-efficient algorithms, ACM Review, Vol. 53, No. 5, pp. 86-96. (2010), doi: 10.1145/1735223.1735245
\bibitem{Albers2010} Albers, S.: Energy-efficient algorithms. Commun. ACM 53(5), 86–96 (2010)

\bibitem{Ittner2007} Barroso, L.A., H\"{o}lzle, U.: The Case for Energy-Proportional Computing. Computer 40(12), 33–37 (2007)

\bibitem{Beloglazov2012} Beloglazov, A., Abawajy, J., Buyya, R.: Energy-aware Resource Allocation Heuristics for Efficient Management of Data Centers for Cloud Computing. Future Generation Computer Systems 28(5), 755–768 (2012)

\bibitem{Beloglazov2011} Beloglazov, A. and Buyya, R.: Optimal Online Deterministic Algorithms and Adaptive Heuristics for Energy and Performance Efficient Dynamic Consolidation of Virtual Machines in Cloud Data Centers, CONCURRENCY AND COMPUTATION: PRACTICE AND EXPERIENCE, Concurrency Computat.: Pract. Exper., pp. 1-24, (2011), doi: 10.1002/cpe

\bibitem{Buyya2009a} Buyya, R., Yeo, C., Venugopal, S., Broberg, J., Brandic, I.: Cloud computing and emerging IT platforms: Vision, hype, and reality for delivering computing as the 5th utility. Future Generation Computer Systems 25(6), 599–616 (2009)

\bibitem{Fan2007a} Fan, X., Weber, W.-D., Barroso, L.A.: Power provisioning for a warehouse-sized computer. ACM SIGARCH Comput. Archit. News. 35, 13 (2007)

%\bibitem{Goiri2010} Goiri, \'{I}., Nou, R., Berral, J., Guitart, J., Torres, J.: Energy-aware Scheduling in Virtualized Datacenters. In: IEEE International Conference on Cluster Computing, CLUSTER 2010, pp. 58–67 (2010)

\bibitem{Hung2011} Quang-Hung, N., Thoai, N., Son, N.T.: Performance constraint and power-aware allocation for user requests in virtual computing lab, Journal of Science and Technology (Vietnam), vol. \textbf{49}, No. 4A, pp. 383-392 (2011.)

%\bibitem{GAPA} Quang-Hung, N., Nien, P. D., Nam, N. H., Tuong, N. H., and Thoai, N..: A Genetic Algorithm for Power-Aware Virtual Machine Allocation in Private Cloud, ICT-EurAsia’13, vol. LNCS \textbf{7804}, pp. 183--191. (2013) doi: 10.1007/978-3-642-36818-9\_19

\bibitem{Hung2013}Quang-Hung, N. et al.: EPOBF: Energy Efficient Allocation of Virtual Machines in High Performance Computing Cloud. J. Sci. Technol. Vietnamese Acad. Sci. Technol. 51, No. 4B, Special on International Conference on Advanced Computing and Applications (ACOMP2013), 173–182 (2013).

\bibitem{HungGPUGA2014} Quang-Hung, N. et al.: A GPU-Based Enhanced Genetic Algorithm for Power-Aware Task Scheduling Problem in HPC Cloud. ICT-EurAsia 2014. LNCS 8407, 159–169 (2014).

\bibitem{Le2011} Le, K. et al.: Reducing electricity cost through virtual machine placement in high performance computing clouds. In: Lathrop, S. et al. (eds.) Proceedings of 2011 International Conference for High Performance Computing, Networking, Storage and Analysis on - SC ’11. p. 1 ACM Press, New York, USA (2011).

\bibitem{Mauch2013} Mauch, V. et al.: High performance cloud computing. Futur. Gener. Comput. Syst. 29, 6, 1408–1416 (2013).

\bibitem{Sotomayor2008} Sotomayor, B., Keahey, K., Foster, I.: Combining batch execution and leasing using virtual machines. In: Proceedings of the Eighteenth International Symposium on High Performance Distributed Computing (HPDC’08), Boston, MA, USA, 23–27 June 2008, pp. 87–96 (2008)

%\bibitem{Sotomayor2009c} Sotomayor, B. and Ignacio, M. and Foster, I.: Resource Leasing and the Art of Suspending Virtual Machines, The 11th IEEE International Conference on High Performance Computing and Communications (HPCC-09),  pp. 59-68. IEEE Computer Society Washington, DC, USA (2009) doi: 10.1109/HPCC.2009.17

\bibitem{Sotomayor2010} Sotomayor, B.: Provisioning Computational Resources Using Virtual Machines and Leases,  PhD Thesis submited to The University of Chicago, US, (2010)

\bibitem{Speitkamp2010} Speitkamp, B., Bichler, M.: A mathematical programming approach for server consolidation problems in virtualized data centers. Serv. Comput. 3, 266–278 (2010)

\bibitem{VonLaszewski2009} von Laszewski, G., Wang, L., Younge, A.J., He, X.: Power-aware scheduling of virtual machines in DVFS-enabled clusters. In: IEEE Intl. Conf. on Cluster Computing and Workshops, 2009, pp. 1–10 (2009), doi:10.1109/CLUSTR.2009.5289182

\bibitem{Panigrahy2011} Panigrahy, R., Talwar, K., Uyeda, L., Wieder, U.: Heuristics for vector bin packing. Technical report, Microsoft Research (2011)

\bibitem{Pham2010} Pham, T.V. et al.: A service composition framework for market-oriented high performance computing cloud. Proceedings of the 19th ACM International Symposium  on High Performance Distributed Computing - HPDC ’10. p. 284 ACM Press, New York, New York, USA (2010).

\bibitem{Feitelson2004} Feitelson, D.G., Rudolph, L., Schwiegelshohn, U.: Parallel job scheduling - a status report. In: Feitelson, D.G., Rudolph, L., Schwiegelshohn, U. (eds.) JSSPP 2004. LNCS, vol. 3277, pp. 1–16. Springer, Heidelberg (2005)

\bibitem{Garg2009} Garg, S.K., Yeo, C.S., Anandasivam, A., Buyya, R.: Energy-Efficient Scheduling of HPC Applications in Cloud Computing Environments. arXiv Prepr. arXiv0909.1146 (2009)

\bibitem{Vis2011} Viswanathan, H. et al.: Energy-Aware Application-Centric VM Allocation for HPC Workloads. 2011 IEEE International Symposium on Parallel and Distributed Processing Workshops and Phd Forum. pp. 890–897 IEEE (2011).

\bibitem{Cloudsim} Calheiros, R.N. et al.: CloudSim: a toolkit for modeling and simulation of cloud computing environments and evaluation of resource provisioning algorithms. Softw. Pract. Exp. 41, 1, 23–50 (2011).

\bibitem{Tako2012} Takouna, I. et al.: Energy efficient scheduling of HPC-jobs on virtualize clusters using host and VM dynamic configuration. ACM SIGOPS Oper. Syst. Rev. 46, 2, 19 (2012).

\bibitem{Maam2011} M\"{a}mmel\"{a}, O. et al.: Energy-aware job scheduler for high-performance computing. Comput. Sci. - Res. Dev. 27, 4, 265–275 (2011).

%\bibitem[Spec1]{Spec1} SPECpower ssj2008 results for Fujitsu Siemens Computers PRIMERGY RX200 S4 (Intel Xeon L5430). \url{http://bit.ly/LvmII4}

%\bibitem{Spec2} SPECpower ssj2008 results for HP ProLiant DL585 G5 (2.70GHz, AMD Opteron 8384). \url{http://bit.ly/JrkskF}

%\bibitem{Spec3} SPECpower ssj2008 results for HP ProLiant DL785 G5 (2.30GHz, AMD Opteron 8376 HE). \url{http://bit.ly/K99RfD}

%\bibitem{SDSC} The San Diego Supercomputer Center (SDSC) Blue Horizon log. \url{http://bit.ly/JUQsiP}
\bibitem{WorkloadLPC} The LPC log from the Parallel Workloads Archive. \url{http://www.cs.huji.ac.il/labs/parallel/workload/l\_lpc/LPC-EGEE-2004-1.2-cln.swf.gz}. Last accessed: 30-January-2014

\bibitem{AmazonEC2HPC}  http://aws.amazon.com/hpc/

\end{thebibliography}


==> results.tex <==
\begin{table}
\centering
\caption{The normalized total energy consumption. Simulation results of scheduling algorithms solving scheduling problems with 12681 VMs and 5000 physical machines (hosts) using Feiltelson's parallel workload model \cite{feitelson1996workloadmodel}}
	\label{table:simresult-feitelsonmodel1000jobs}
\begin{tabular}{|l|c|c|c|c|}
\hline
Algorithms   & \multicolumn{1}{l|}{\#Hosts} & \multicolumn{1}{l|}{\#VMs} & \multicolumn{1}{l|}{Energy (KWh)} & \multicolumn{1}{l|}{Norm. Energy} \\ \hline
PABFD        & 5000                         & 12681                      & 1,055.42                    & 1.598                            \\ \hline
VBP-Norm-L2  & 5000                         & 12681                      & 1,054.69                    & 1.597                            \\ \hline
Tian-MFFDE   & 5000                         & 12681                      & 660.30                      & 1.000                            \\ \hline
MinDFT-LDTF  & 5000                         & 12681                      & 603.90                      & 0.915                            \\ \hline
MinDFT-LFT   & 5000                         & 12681                      & 503.43                      & 0.762                            \\ \hline
EMinTRE-LDTF & 5000                         & 12681                      & 496.55                      & 0.752                            \\ \hline
\end{tabular}
\end{table}

\begin{table}
	\centering
	\caption{The normalized total energy consumption. Simulation results of scheduling algorithms solving scheduling problems with 29,177 VMs and 10,000 physical machines (hosts) using Feiltelson's parallel workload model \cite{feitelson1996workloadmodel}}
	\label{table:simresult-feitelsonmodel2000jobs}
	\begin{tabular}{|l|c|c|c|c|}
		\hline
		Algorithms   & \multicolumn{1}{l|}{\#Hosts} & \multicolumn{1}{l|}{\#VMs} & \multicolumn{1}{l|}{Energy (KWh)} & \multicolumn{1}{l|}{Norm. Energy} \\ \hline
		PABFD        & 10000                        & 29177                      & 2261.878                          & 1.540                                  \\ \hline
		VBP-Norm-L2  & 10000                        & 29177                      & 2260.615                          & 1.539                                  \\ \hline
		Tian-MFFDE   & 10000                        & 29177                      & 1468.409                          & 1.000                                  \\ \hline
		MinDFT-LDTF  & 10000                        & 29177                      & 1373.764                          & 0.936                                  \\ \hline
		MinDFT-LFT   & 10000                        & 29177                      & 1109.852                          & 0.756                                  \\ \hline
		EMinTRE-LDTF & 10000                        & 29177                      & 1092.365                          & 0.744                                  \\ \hline
	\end{tabular}
\end{table}

\begin{table}
	\centering
	\caption{The normalized total energy consumption. Simulation results of scheduling algorithms solving scheduling problems with 8847 VMs and 5000 physical machines (hosts) using Lublin99's parallel workload model \cite{lublin2003workload}}
	\label{table:simresult-lublin99model1000jobs}
	\begin{tabular}{|l|c|c|c|c|}
		\hline
		Algorithms   & \multicolumn{1}{l|}{\#Hosts} & \multicolumn{1}{l|}{\#VMs} & \multicolumn{1}{l|}{Energy (KWh)} & \multicolumn{1}{l|}{Norm. Energy} \\ \hline
	PABFD        & 5000                       & 8847                     & 460.664                                 & 1.601                                  \\ \hline
	VBP-Norm-L2  & 5000                       & 8847                     & 453.229                                 & 1.575                                  \\ \hline
	Tian-MFFDE   & 5000                       & 8847                     & 287.779                                 & 1.000                                  \\ \hline
	MinDFT-LDTF  & 5000                       & 8847                     & 263.860                                 & 0.917                                  \\ \hline
	MinDFT-LFT   & 5000                       & 8847                     & 232.286                                 & 0.807                                  \\ \hline
	EMinTRE-LDTF & 5000                       & 8847                     & 220.675                                 & 0.767                                  \\ \hline
	\end{tabular}
\end{table}

\begin{table}
	\centering
	\caption{The normalized total energy consumption. Simulation results of scheduling algorithms solving scheduling problems with 19853 VMs and 5000 physical machines (hosts) using Lublin99's parallel workload model \cite{lublin2003workload}}
	\label{table:simresult-lublin99model2000jobs}
	\begin{tabular}{|l|c|c|c|c|}
		\hline
		Algorithms   & \multicolumn{1}{l|}{\#Hosts} & \multicolumn{1}{l|}{\#VMs} & \multicolumn{1}{l|}{Energy (KWh)} & \multicolumn{1}{l|}{Norm. Energy} \\ \hline
		PABFD        & 5000                         & 19853                      & 3107.78                           & 1.424                                  \\ \hline
		VBP-Norm-L2  & 5000                         & 19853                      & 3106.56                           & 1.423                                  \\ \hline
		Tian-MFFDE   & 5000                         & 19853                      & 2182.54                           & 1.000                                  \\ \hline
		MinDFT-LDTF  & 5000                         & 19853                      & 1927.52                           & 0.883                                  \\ \hline
		MinDFT-LFT   & 5000                         & 19853                      & 1746.12                           & 0.800                                  \\ \hline
		EMinTRE-LDTF & 5000                         & 19853                      & 1485.13                           & 0.680                                  \\ \hline
	\end{tabular}
\end{table}
